A Consistent Bayesian Formulation for Stochastic Inverse Problems Based on Push-forward Measures

We formulate, and present a numerical method for solving, an inverse problem for inferring parameters of a deterministic model from stochastic observational data (quantities of interest). The solution, given as a probability measure, is derived using a Bayesian updating approach for measurable maps that finds a posterior probability measure, that when propagated through the deterministic model produces a push-forward measure that exactly matches the observed probability measure on the data. Our approach for finding such posterior measures, which we call consistent Bayesian inference, is simple and only requires the computation of the push-forward probability measure induced by the combination of a prior probability measure and the deterministic model. We establish existence and uniqueness of observation-consistent posteriors and present stability and error analysis. We also discuss the relationships between consistent Bayesian inference, classical/statistical Bayesian inference, and a recently developed measure-theoretic approach for inference. Finally, analytical and numerical results are presented to highlight certain properties of the consistent Bayesian approach and the differences between this approach and the two aforementioned alternatives for inference.

==> max-entropy.tex <==
%In this paper we will consider the process of updating prior belief about model parameters, in the form of a probability distribution, when new data that constrains the prior belief becomes available. Bayesian and maximum entropy methods are two popular updating methods.

Bayesian methods~\cite{Kaipio_S_ACIP_2007,Stuart_IP_2010} are the most popular means of infering probabilistic descriptions of model parameters from data. Conceptually Bayesian methods provide a means
of updating prior belief, in the form on a probability distribution, when new information becomes available. Given data $d$ and model parameters $\lambda$, Bayes theorem states that the updated parameter distribution, the posterior $\pi(\lambda|d)$, is proportional to the product of the prior distribution on the model parameters $\pi(\lambda)$ and the assumed relationship between the data and the model parameters known as the likelihood $\pi(d|\lambda)$, i.e. $\pi(\lambda|d)\propto\pi(\lambda)\pi(d|\lambda)$.

The
prior knowledge or belief about $\lambda$ is codified both into the prior
$\pi(\lambda)$ and also in the likelihood function $\pi(d|\lambda)$.
The selection of the prior is a contentious issue and has given rise to a number of approaches, such as robust Bayesian inference and maximum entropy methods that attempt to address this issue. Robust Bayesian inference~\cite{Berger_TEST_1994} is the study of the sensitivity of Bayesian posteriors to the uncertain components of the Bayesian analysis, typically the prior and the likelihood function. Maximum entropy methods~\cite{Caticha_P_PRE_2004,Gull_Chapter_1988} choose the prior to be the probability density that maximizes entropy, whilst respecting any specified constraints. For example if only the mean and variance of the prior are known then the density that maximizes entropy is the Gaussian distribution.

